Assessing the Quality of a Set of Basis Functions for Inverse Optimal Control via Projection onto Global Minimizers

Inverse optimization (Inverse optimal control) is the task of imputing a cost function such that given test points (trajectories) are (nearly) optimal with respect to the discovered cost. Prior methods in inverse optimization assume that the true cost is a convex combination of a set of convex basis functions and that this basis is consistent with the test points. However, the consistency assumption is not always justified, as in many applications the principles by which the data is generated are not well understood. This work proposes using the distance between a test point and the set of global optima generated by the convex combinations of the convex basis functions as a measurement for the expressive quality of the basis with respect to the test point. A large minimal distance invalidates the set of basis functions. The concept of a set of global optima is introduced and its properties are explored in unconstrained and constrained settings. Upper and lower bounds for the minimum distance in the convex quadratic setting are implemented by bi-level gradient descent and an enriched linear matrix inequality respectively. Extensions to this framework include max-representable basis functions, nonconvex basis functions (local minima), and applying polynomial optimization techniques.

==> section-notation.tex <==
\subsection{Notation}
The set of real numbers is $\R$, the $n$-dimensional Euclidean space is $\R^n$, and its nonnegative real orthant is $\R^n_+$. The vector of all zeros is $0$ and of all ones is $\mathbf{1}$. The set of natural numbers (incl. 0) is $\N$, and its subset between $1$ and $N$ is $1..N$. The $n$-dimensional probability simplex is $\Delta^n$.  The set of $m\times n$ real-valued matrices is $\R^{m \times n}$. The set of $n\times n$ symmetric real matrices satisfying $Q = Q^T$ is $\psd^n$.
A symmetric matrix is \ac{PSD} $(Q \in \psd^n_+)$ if $\forall x \in \R^n: \ x^T Q x \geq 0$, and is \ac{PD} $(Q \in \psd^n_{++})$ if $\forall x \in \R^n, x \neq 0: x^T Q x > 0$.

Let $X$ and $Y$ be a pair of spaces. A single valued function may be written as $f:X \rightarrow Y$, and a set valued function $F: 2^X \rightarrow 2^Y$ may be expressed as $F: X \rightrightarrows Y$.
The projection $\pi^x: (x, y) \mapsto x$ operation applied to a set $\hat{\mathbb{J}} \subseteq X \times Y$ is, 
\begin{equation}
    \mathbb{J}(x) = \pi^x \hat{\mathbb{J}}(x,y) = \{x \mid \exists y \in Y: (x, y) \in \hat{\mathbb{J}}\}.
\end{equation}
